Simulations of Bosonic BMN Matrix Model

In this thesis we provide the results obtained through lattice Monte Carlo simulations of the bosonic BMN and the bosonic BFSS matrix models. The simulations are performed using Hybrid Monte Carlo (HMC) algorithm. The BMN matrix model is expected to have a Hagedorn/deconfinement type phase transition as the temperature is varied in the system. The Polyakov loop is used as an order parameter for detecting the phase transition. Besides the Polyakov loop, other prime observables such as the internal energy and the extent of space were also computed. We also check the validity of numerical simulation algorithms by exploring the behavior of various relevant toy models. As the main result of this thesis, we present a parametrized phase diagram of the bosonic BMN matrix model constructed using two dimensionless parameters: a dimensionless coupling constant and a dimensionless temperature.

==> nota.tex <==
\begin{center}
\LARGE{ \bf Notation and Abbreviations}  
\end{center}

\begin{center}
\begin{tabular}{l l}
$\theta_{i,j}$ & Weight matrix \\ 
$b_j$ & Biased term for each layer\\
$F_i$ & Activation function of $i^{th}$ layer\\
ROE & Rest of Events\\
MVA & Multivariate Analysis\\
BDT & Boosted Decision Tree\\
DNN & Deep Neural Network\\
TMVA & Toolkit for Multivariate Analysis\\
ROC & Receiver Operating Curve\\
GPU & Graphical Processing Unit\\
%$\mathbb{F_i}$ & Activation function of $i^{th}$ layer\\
\end{tabular} 
\end{center}

